Diverse features of dust particles and their aggregates inferred from experimental nanoparticles

Nanometre- to micrometre-sized solid dust particles play a vital role in star and planet formations. Despite of their importance, however, our understanding of physical and chemical properties of dust particles is still provisional. We have conducted a condensation experiment of the vapour generated from a solid starting material having nearly cosmic proportions in elements. A laser flash heating and subsequent cooling has produced a diverse type of nanoparticles simultaneously. Here we introduce four types of nanoparticles as potential dust particles in space: amorphous silicate nanoparticles (type S); core/mantle nanoparticles with iron or hydrogenised-iron core and amorphous silicate mantle (type IS); silicon oxycarbide nanoparticles and hydrogenised silicon oxycarbide nanoparticles (type SiOC); and carbon nanoparticles (type C), all produced in a single heating-cooling event. Type IS and SiOC nanoparticles are new for potential astrophysical dust. The nanoparticles are aggregated to a wide variety of structures, from compact, fluffy, and networked. A simultaneous formation of nanoparticles, which are diverse in chemistry, shape, and structure, prompts a re-evaluation of astrophysical dust particles

==> references.tex <==
@article{Anders1987,
author={Anders, E.},
title={Local and Exotic Components of Primitive Meteorites, and their Origin},
journal={Phil. Trans. R. Soc. Lond. A},
fjournal={Philosophical Transactions of the Royal Society of London. Series A},
volume=323,
pages={287-304},
year=1987,
doi={https://doi.org/10.1098/rsta.1987.0086}
}


@article{Bazell1990,
author={Bazell, D. and Dwek, E.},
title={The Effects of Compositional Inhomogeneities and Fractal Dimension on the Optical Properties of Astrophysical Dust},
journal={ApJ.},
fjournal={Astrophysical Journal},
volume=360,
pages={142},
year=1990,
doi={https://ui.adsabs.harvard.edu/link_gateway/1990ApJ...360..142B/doi:10.1086/169104}
}

@article{Bundy1967,
author={Bundy, F. P. and Kasper, J. S.},
title={Hexagonal Diamond - A New Formation of Carbon},
journal={J. Chem. Phys.},
fjournal={The journal of Chemical Physics},
volume=46,
pages={3437},
year=1967,
doi={https://doi.org/10.1063/1.1841236}
}

@article{Bilalbegovic2017,
author={Bilabegovi\'{c}, G. and Maksimovi\'{c}, A. and Moha\^{c}ek-Gro\^{s}ev, V.},
title={Missing Fe: hydrogenated iron nanoparticles},
journal={MNRAS},
fjournal={Monthly Notices of the Royal Astronomical Society},
volume=466,
pages={L14-L18},
year=2017,
doi={https://doi.org/10.1093/mnrasl/slw226}
}

@article{Birnstiel2016,
author={Birnstiel, T. and Fang, M. and Johansen, A.},
title={Dust Evolution and the Formation of Planetesimals},
journal={Space Sci. Rev.},
fjournal={Space Science Reviews},
volume=205,
pages={41-75},
year=2016,
doi={https://doi.org/10.1007/s11214-016-0256-1}
}


@article{Carrol1976,
author={Carroll, P. J. and McCormack, P. and Oconnor, S.},
title={Iron hydride: loboratory studies and solar identification},
journal={ApJ.},
fjournal={Astrophyusical Journal},
volume=208,
pages={903-913},
year=1976,
doi={hhttps://ui.adsabs.harvard.edu/link_gateway/1976ApJ...208..903C/doi:10.1086/154679}
}


@article{Castleman1988,
author={Castleman Jr., A. W. and Keesee, R. G.},
title={Gas-Phase Clusters: Spanning the States of Matter},
journal={Science},
fjournal={Science},
volume=241,
pages={36-42},
year=1988,
doi={https://doi.org/10.1126/science.241.4861.36}
}


@article{Dorschner1995,
author={Dorschner, J. and Henning, T.},
title={Dust metamorphosis in the galaxy},
journal={The Astron Astrophys Rev},
fjournal={The Astronomy and Astrophysics Review},
volume=6,
pages={271-333},
year=1995,
doi={https://doi.org/10.1007/BF00873686}
}

@book{Draine1990,
author={Draine, B. T.},
title={Evolution of intersetllar dust},
publisher={Astronomical Society of the Pacific},
  booktitle={Proceedings of the Conference: 1989},
pages={193-205},
year=1990,
}

@article{Dwek2016,
author={Dwek, E.},
title={IRON: A KEY ELEMENT FOR UNDERSTANDING THE ORIGIN AND EVOLUTION OF INTERSTELLAR DUST},
journal={ApJ.},
fjournal={The Astrophysical Journal},
volume=825,
pages={136},
year=2016,
doi={https://iopscience.iop.org/article/10.3847/0004-637X/825/2/136}
}


@article{Ehrenfreund2010,
author={Ehrenfreund, P. and Cami, J.},
title={Cosmic Carbon Chemistry: From the Interstellar Medium to the Early Earth},
journal={Cold Spring Harbor Perspectives in Bilogy},
fjournal={Cold Spring Harbor Perspectives in Bilogy},
volume=2,
pages={a002097},
year=2010,
doi={10.1101/cshperspect.a002097}
}



@article{Flagan1995,
author={Flagan, R. C. and Lunden, M. M.},
title={Particle structure control in nanoparticle synthesis form the vapor phase},
journal={Mater. Sci. Eng. A.},
fjournal={Materials Science and Engineering: A},
volume=204,
pages={113-124},
year=1995,
doi={https://doi.org/10.1016/0921-5093(95)09947-6}
}

@article{Granqvist1976,
author={Granquvist, C. G. and Buhrman, R. A.},
title={Ultrafine metal particles},
journal={J. Appl. Phys.},
fjournal={Journal of Applied Physics},
volume=47,
pages={2200-2219},
year=1976,
doi={https://doi.org/10.1063/1.322870}
}


@book{Greenberg1989,
author={Greenberg, J. M.},
title={The core-mantle model of intersetllar grains and the cosmic dust connection},
publisher={Kluwer Academic Publishers},
  booktitle={Proceedings of the 135th Symposium of the International Astronomical Union: 1988},
pages={345-355},
year=1989,
url={https://adsabs.harvard.edu/full/1989IAUS..135..345G}
}

@article{Huss1995,
author={Huss, G. R. and Lewis, R. S.},
title={Presolar diamond, SiC, and graphite in primitive chondrites: Abundances as a function of meteorite class and petrologic type},
journal={GCA},
fjournal={Geochimica et Cosmochimica Acta},
volume=59,
pages={115-160},
year=1995,
doi={https://doi.org/10.1016/0016-7037(94)00376-W}
}


@article{Henning2010,
author={Henning, Th.},
title={Cosmic silicates},
journal={Annu. Rev. Astron. Astrophys.},
fjournal={Annual Review of Astronomy and Astrophysics},
volume=48,
pages={21-46},
year=2020,
doi={https://doi.org/10.1146/annurev-astro-081309-130815}
}

@article{Hensley2021,
author={Hensley, B. S. and Draine, B. T.},
title={Observational Constraints on the Physical Properties of Interstellar Dust in the Post-Plank Era},
journal={ApJ},
fjournal={The Astrophysical Journal},
volume=906,
pages={73},
year=2021,
doi={https://doi.org/10.3847/1538-4357/abc8f1}
}

@article{Jager1994,
author={J\"ager, C. and Mutschke, H. and Begemann, B. and Dorschner, J. and Henning, Th.},
title={Steps toward interstellar silicate mineralogy. I. Laboratory results of a silicate glass of mean cosmic composition},
journal={A\&A},
fjournal={Astronomy and Astrophysics},
volume=292,
pages={641-655},
year=1994,
doi={https://articles.adsabs.harvard.edu/pdf/1994A\%26A...292..641J}
}

@article{Jager1998,
author={J\"ager, C. and Molster, J. and Dorschner, J. and Henning, Th. and Mutschke, H. and Waters L. B. F. M.},
title={Steps toward interstellar silicate mineralogy. IV. The crystalline revolution},
journal={A\&A},
fjournal={Astronomy and Astrophysics},
volume=339,
pages={904-916},
year=1998,
doi={https://articles.adsabs.harvard.edu/cgi-bin/nph-iarticle_query?1998A\%26A...339..904J&defaultprint=YES&filetype=.pdf}
}


@article{Jarosewich1990,
author={Jarosewich, E.},
title={Chemical analyses of meteorites: A compilation of stony and iron meteorite analyses},
journal={Meteoritics},
fjournal={Meteoritics},
volume=25,
pages={323-337},
year=1990,
doi={https://doi.org/10.1111/j.1945-5100.1990.tb00717.x}
}


@article{Johnson1988,
author={Johnson, H. H.},
title={Hydrogen in Iron},
journal={Metall. Trans. B},
fjournal={Metallurgical Transactions B},
volume=19,
pages={691-707},
year=1988,
doi={https://link.springer.com/content/pdf/10.1007/BF02650189.pdf}
}

@article{Jones1994,
author={Jones, A. P. and Tielens, A. G. G. M. and Hollenbarch, D. J. and McKee, C. F.},
title={Grain Desruction in Shocks in the Intersetllar Medium},
journal={ApJ},
fjournal={Astrophysical Journal},
volume=433,
pages={797-810},
year=1994,
doi={https://articles.adsabs.harvard.edu/pdf/1994ApJ...433..797J}
}

@article{Jones1996,
author={Jones, A. P. and Tielens, A. G. G. M. and Hollenbarch, D. J. },
title={Grain Shattering in Shocks: The Interstellar Grain Size Distribution},
journal={ApJ},
fjournal={Astrophysical Journal},
volume=469,
pages={740-764},
year=1996,
doi={https://articles.adsabs.harvard.edu/pdf/1996ApJ...469..740J}
}

@book{Jones2004,
author={Jones, A. P.},
title={Dust Destruction Processes},
publisher={Vol. 309, Proceedings of the conference held 26-30 May},
  booktitle={Astrophysics of Dust, ASP Conference Series, },
pages={347},
year=2004,
url={}
}


@article{Jones2011,
author={Jones, A. P. and Nuth III, J. A.},
title={Dust destruction in the ISM: a re-evaluation of dust lifetimes},
journal={A\&A},
fjournal={Astronomy and Astrophysics},
volume=530,
pages={A44},
year=2011,
doi={https://doi.org/10.1051/0004-6361/201014440}
}


@article{Krasnokutski2017,
author={Krasnokutski, S. A. and Goulart, M. and Gordon, E. B. and Ritsch, A. and J\"ager, C. and Rastogi, M. and Salvenmoser, W. and Henning, Th. and Scheier, P.},
title={Low-TEmperature Condensation of Carbon},
journal={ApJ.},
fjournal={The Astrophyical Journal},
volume=847,
pages={89},
year=2017,
doi={10.3847/1538-4357/aa88a4}
}


@article{Kim1995,
author={Kim, S-H. and Martin, P. G.},
title={Particles as Determined from Polarization: Spheroids},
journal={ApJ.},
fjournal={Astrophysical Jouranl},
volume=444,
pages={293},
year=1995,
doi={https://ui.adsabs.harvard.edu/link_gateway/1995ApJ...444..293K/doi:10.1086/175604}
}


@article{Kimoto1963,
author={Kimoto, K. and Kamiya, Y. and Nonoyama, M. and Uyeda, R.},
title={An Electron Microscope Study on Fine Metal Particles Prepared by Evaporation in Argon Gas at Low Pressure},
journal={Jpn. J. App. Phys.},
fjournal={Japanese Journal of Applied Physics},
volume=2,
pages={702-713},
year=1963,
doi={https://doi.org/10.1143/JJAP.2.702}
}

@article{Kimura2017,
author={Kimura, Y. and Tanaka, K. K. and Nozawa, T. and Takeuchi, S. and Inatomi, Y.},
title={Pure iron grains are in the universe},
journal={Sci. Adv.},
fjournal={Science advance},
volume=3,
pages={e1601992},
year=2017,
doi={https://www.science.org/doi/10.1126/sciadv.1601992}
}


@article{Kimura2022,
author={Kimura, Y. and Tanaka, K. K. and Inatomi, Y. and Ferguson, F. T. and Nuth III, J. A.},
title={Inefficient Growth of SiOx Grains: Implications for Circumsttellar Outflows},
journal={ApJ},
fjournal={The Astrophysical Jouranl Letters},
volume=934,
pages={eL10},
year=2022,
doi={https://iopscience.iop.org/article/10.3847/2041-8213/ac8002}
}


@article{Kimura2023,
author={Kimura, Y. and Tanaka, K. K. and Inatomi, Y. and Aktas, C. and Blum, J.},
title={Nucleation experiments on a titanium-carbon system imply nonclassical formation of presolar grains},
journal={Science Advances},
fjournal={Science Advances},
volume=9,
pages={eadd8295},
year=2023,
doi={https://doi.org/10.1126/sciadv.add8295}
}


@article{Kozasa1992,
author={Kozasa, T. and Blum, J. and Mukai, T.},
title={Optical properties of dust aggregates. I - Wavelength dependence},
journal={ApJ.},
fjournal={Astrophysical Jouranl},
volume=263,
pages={423-432},
year=1992,
doi={https://adsabs.harvard.edu/full/1992A%26A...263..423K}
}

@article{Kuramoto1996,
author={Kuramoto, K. and Matsui, T.},
title={Partitioning of H and C between the mantle and core during the core formation in the Earth: Its implications for the atmospheric evolution and redox state of early mantle},
journal={JGR},
fjournal={Jouranl of Geophysical Research},
volume=101,
pages={909-932},
year=1996,
doi={https://doi.org/10.1029/96JE00940}
}

@article{Lecuyeri1998,
author={Lecuyer, C. and Gillet, P. and Robert, F.},
title={The hydrogen isotope composition of seawater and the global water cycle},
journal={Che. Geol.},
fjournal={Chemical Geology},
volume=145,
pages={249-261},
year=1998,
doi={https://doi.org/10.1016/S0009-2541(97)00146-0}
}

@article{Linsky1998,
author={Linsky, J.L.},
title={Deuterium abundance in the local ism and possible spatial variations.},
journal={Space Sci. Rev.},
fjournal={Space Science Review},
volume=84,
pages={285-296},
year=1998,
doi={https://doi.org/10.1023/A:1005048124341}
}

@article{Hashimoto2021,
author={Hashimoto, A. and Nakano, Y.},
title={Bubbles to Chondrite-II. Chemical fractionations in chondrites.},
journal={Prog. Earth Planet. Sci.},
fjournal={Progress Earth Planetary Science},
volume=8,
pages={9},
year=2021,
doi={https://doi.org/10.1186/s40645-020-00382-8}
}



@article{Li1997,
author={Li, A. and Greenberg, J. M.},
title={A unified model of intersetllar dust},
journal={A\&A},
fjournal={Astronomy and Astrophysics},
volume=323,
pages={566-584},
year=1997,
doi={https://adsabs.harvard.edu/full/1997A\%26A...323..566L}
}


@article{Mathis1977,
author={Mathis, J. S. and Rumpl, W. and Nordsieck, K. H.},
title={The size distribution of interstellar grains},
journal={ApJ},
fjournal={Astrophyical Journal},
volume=217,
pages={425-433},
year=1977,
doi={https://ui.adsabs.harvard.edu/link_gateway/1977ApJ...217..425M/doi:10.1086/155591}
}

@article{Mathis1989,
author={Mathis, J. S. and Whiffen, G.},
title={Composite interstellar grains},
journal={ApJ},
fjournal={Astrophyical Journal},
volume=341,
pages={808-822},
year=1989,
doi={https://adsabs.harvard.edu/pdf/1989ApJ...341..808M}
}

@article{Mathis1990,
author={Mathis, J. S.},
title={Intersetllar Dust and Extinction},
journal={Annu. Rev. Astron. Astrophys.},
fjournal={Astronomy and Astrophysics},
volume=28,
pages={37-70},
year=1990,
doi={https://doi.org/10.1146/annurev.aa.28.090190.000345}
}



@article{Meakin1988,
author={Meakin, P.},
title={TFractal aggregates},
journal={ Adv. Colloid Interface Sci.},
fjournal={Advances in Colloid and Interface Science},
volume=228,
pages={249-331},
year=1988,
doi={https://doi.org/10.1016/0001-8686(87)80016-7}
}

@article{Mould1978,
author={Mould, J. R. and Wyckoff, S.},
title={Iron hydride in stellar atmospheres},
journal={MNRAS},
fjournal={Monthly Notices of the Royal Astronomical Society},
volume=182,
pages={63-68},
year=1978,
doi={https://doi.org/10.1093/mnras/182.1.63}
}

@article{Mukai1992,
author={Mukai, T. and Ishimoto, H. and Kozasa, T. and Blum, J. and Greenberg, J. M.},
title={Radiation pressure forces of fluffy porous grains},
journal={A\$A},
fjournal={Astronomy and Astrophysics},
volume=262,
pages={315-320},
year=1992,
doi={https://articles.adsabs.harvard.edu/cgi-bin/nph-iarticle_query?1992A\%26A...262..315M&defaultprint=YES&filetype=.pdf}
}

@article{Nakano2023,
author={Nakano, Y. and Kimura, Y. and Hashimoto, A.},
title={Characterization of potentially-interstellar, nanoparticles condensed in hydrogen atmosphere},
journal={54th LPSC abstract},
fjournal={54th Lunar and Planetary Science Conference 2023},
volume=2806,
pages={},
year=2023,
doi={https://www.hou.usra.edu/meetings/lpsc2023/pdf/1296.pdf}
}

@article{Nakano2020,
author={Nakano, Y. and Hashimoto, A.},
title={Bubbles to Chondrites-I. Evaporation and condensation experiments, and formation of chondrules},
journal={Prog. Earth Planet Sci.},
fjournal={Progress in Earth and Planetary Science},
volume=7,
pages={47},
year=2020,
doi={https://doi.org/10.1186/s40645-020-00335-1}
}


@book{Natta2007,
author={Natta, A. and Testi, L. and Calvet, H. and Henning, Th. and Waters, R. and Wilner, D.},
title={Dust in Protoplanetary Disks: Propeties and Evolutions},
publisher={University of Arizona Press, Tucson},
  booktitle={Protostars and Planets V, Reipurth B., Jewitt, D., Keil K.,},
pages={767-781},
year=2007,
url={https://ui.adsabs.harvard.edu/abs/2007prpl.conf..767N/abstract}
}


@article{Okuchi1997,
author={Okuchi, T.},
title={Hydroen Partitioning into Molten Iron at High Pressure: Implicattions for Earth's Core},
journal={Science},
fjournal={Science},
volume=278,
pages={1781-1784},
year=1997,
doi={https://doi.org/10.1126/science.278.5344.1781}
}

@article{Okuchi1998,
author={Okuchi, T.},
title={The melting temperature of iron hydride at high pressures and its implications for the temperature of the Earth's core},
journal={J. Phys.: Condens. Matter.},
fjournal={Journal of Physics: Condensed Matter},
volume=10,
pages={11595},
year=1998,
doi={https://iopscience.iop.org/article/10.1088/0953-8984/10/49/052}
}


@article{Pantano1999,
author={Pantano, C. G. and Singh, A. K. and Zhang, H.},
title={Silicon Oxycarbide Glasses},
journal={Journal of Sol-Gel Science and Technology},
fjournal={Journal of Sol-Gel Science and Technology},
volume=14,
pages={7-25},
year=1999,
doi={https://link.springer.com/article/10.1023/A:1008765829012}
}

@article{Potapov2022,
author={Potapov, A. and Bouwman, J.},
title={Importance of laboratory experimental studies of silicate grains for exoplanet atmosphere characterization},
journal={Front. Astron. Space Sci.},
fjournal={Frontiers in Astronomy and Space Sciences},
volume=9,
pages={7-25},
year=2022,
doi={https://doi.org/10.3389/fspas.2022.912302}
}

@article{Richtsmeier1985,
author={Richtsmeier, S. C. and Parks, E. K. and Liu, E. K. and Pobo, L. G. and Riley, S. J.},
title={Gas phase reactions of iron clusters with hydrogen. I. Kinetics},
journal={J. Chem. Phys.},
fjournal={The Journal of Chemical Physics},
volume=82,
pages={3659-3665},
year=21985,
doi={https://doi.org/10.1063/1.448901}
}


@article{Rouille2014,
author={Rouilie, G. and J\"ager, C. and Krasnokutski, S. A. and Krebsz, M. and Henning, Th.},
title={Cold condensation of dust in the ISM},
journal={Faraday Discussions},
fjournal={Faraday Discussions},
volume=168,
pages={449-460},
year=2014,
doi={https://doi.org/10.1039/C4FD00010B}
}

@article{Savage1979,
author={Savage, B. D. and Mathis, J. S.},
title={Observed Properties of Interstellar Dust},
journal={Annu.Rev.Astron. Astrophys.},
fjournal={Annual Review of Astronomy and Astrophysics},
volume=17,
pages={73-111},
year=1979,
doi={https://doi.org/10.1146/annurev.aa.17.090179.000445}
}

@article{Savage1979a,
author={Savage, B. D. and Bohlin, R. C.},
title={The depletion of iterstellar gaseous iron},
journal={ApJ.},
fjournal={Astrophysical Jouranl},
volume=229,
pages={136-146},
year=1979,
doi={https://ui.adsabs.harvard.edu/link_gateway/1979ApJ...229..136S/doi:10.1086/156938}
}

@article{Scheafer1990,
author={Scheafer, D. W. and Hurd, A. J.},
title={Growth and Structure of Combustion Aerosols:
Fumed Silica},
journal={Aerosol Science and Technology},
fjournal={Aerosol Science and Technology},
volume=12,
pages={876-890},
year=1990,
doi={https://doi.org/10.1080/02786829008959400}
}

@article{Siebenmorgen2014,
author={Siebenmorgen, R. and Voshchinnikov, N. V. and Bagnulo, S.},
title={Dust in the diffuse interstellar medium Extinction, emission, linear and circular polarisation},
journal={A\&A},
fjournal={Astronomy and Astrophysics},
volume=561,
pages={A82},
year=2014,
doi={https://doi.org/10.1051/0004-6361/201321716}
}

@article{Stephens1978,
author={Stephens, J. R. and Kothari, B. K.},
title={Laboratory analogues to cosmic dust},
journal={The moon and the planets},
fjournal={The moon and the planets},
volume=19,
pages={139-152},
year=1978,
doi={https://doi.org/10.1007/BF00896984}
}

@article{Stracke2012,
author={Stracke, A. and Palme, H. and Gellissen, M. and M\"unker, C. and Kleine, T. and Birbaum, K. and G\"unther, D. and Bourdon, B.},
title={Refractory element fractionation in the Allende meteorite: Implications for solar nebula condensation and the chondritic composition of planetary bodies},
journal={GCA},
fjournal={Geochimica et Cosmochimica Acta},
volume=85,
pages={114-141},
year=2012,
doi={https://doi.org/10.1016/j.gca.2012.02.006}
}

@article{Sun2023,
author={Sun, S. and He. Y. and Yang, J. and Lin, Y. and Li, J. and Kim, D. Y. and Li, H. and Mao, H-K.},
title={Superionic effect and anisotropic texture in Earth’s inner core driven by geomagnetic field},
journal={Nat. Comm.},
fjournal={Nature Communications},
volume=14,
pages={1656},
year=2023,
doi={https://www.nature.com/articles/s41467-023-37376-1}
}


@article{Takahashi2013,
author={Takahashi, K. and Isobe, S. and Ohnuki, S.},
title={Chemisorption of hydrogen on Fe clusters through hybrid bonding mechanisms},
journal={Appl. Phys. Lett.},
fjournal={Applied Physics Letters},
volume=102,
pages={113108},
year=2013,
doi={https://doi.org/10.1063/1.4798511}
}



@article{Tavakoli2015,
author={Tavakoli, A. H. and Armentrout, M. M. and Sen, S. and Navrotsky, A.},
title={Hydrogenated Si–O–C nanoparticles: Synthesis, structure, and thermodynamic stability},
journal={Journal of Materials Research},
fjournal={Journal of Materials Research},
volume=30,
pages={295-303},
year=2015,
doi={https://doi.org/10.1557/jmr.2014.376}
}

@article{Tennyson2012,
author={Tennyson, J. and Yurchenko, S. N.},
title={ExoMol: molecular line lists for exoplanet and other atmopsheres},
journal={MNRAS},
fjournal={Monthly Notices of the Royal Astronomical Society},
volume=425,
pages={21-33},
year=2012,
doi={https://doi.org/10.1111/j.1365-2966.2012.21440.x}
}


@article{Tielens1998,
author={Tielens, A. G. G. M. and Waters, L. B. F. M. and Molster, F. J. and Justtanont, J.},
title={Circumstellar Silicate Mineralogy},
journal={Astrophysics and Space Science},
fjournal={Astrophysics and Space Science},
volume=255,
pages={415-426},
year=1998,
doi={https://ui.adsabs.harvard.edu/link_gateway/1998Ap&SS.255..415T/doi:10.1023/A:1001585120472}
}



@article{Tielens2022,
author={Tielens, A. G. G. M.},
title={Dust Formation in Astrophysical Environments: The Importance of Kinetics},
journal={Front. Astron. Space Sci.,},
fjournal={Frontiers in Astronomy and Space Sciences},
volume=9,
pages={908217},
year=2022,
doi={https://doi.org/10.3389/fspas.2022.908217}
}


@article{Tohno1996,
author={Tohno, S. and Itoh, M. and Aono, S. and Takano, H.},
title={Production of Contact-Free Nanoparticles by Aerosol Process: Dependence of Particle Size on Gas Pressure},
journal={Journal of Colloid and Interface Science},
fjournal={Journal of Colloid and Interface Science},
volume=180,
pages={574-577},
year=1996,
doi={https://doi.org/10.1006/jcis.1996.0338}
}


@article{Vekilov2019,
author={Vekilov, P. G.},
title={Crystallization tracked atom by atom},
journal={Nature},
fjournal={Nature},
volume=570,
pages={450-452},
year=2019,
doi={https://doi.org/10.1038/d41586-019-01965-2}
}



@article{Wada1968,
author={Wada, N.},
title={Preparation of Fine Metal Particles by Means of Evaporation in Xenon Gas},
journal={Jpn. J. App. Phys.},
fjournal={Japanese Journal of Applied Physics},
volume=180,
pages={574-577},
year=1996,
doi={https://iopscience.iop.org/article/10.1143/JJAP.7.1287}
}



@article{Whetten1985,
author={Whetten, R. L. and Cox, D. M. and Trevor, D. J. and Kaldor, A.},
title={Correspondence between Electron Binding Energy and Chemisorption Reactivity of Iron Clusters},
journal={Phys. Rev. Lett.},
fjournal={Physical Review Letters},
volume=54,
pages={1494},
year=1985,
doi={https://doi.org/10.1103/PhysRevLett.54.1494}
}



@article{Williams1992,
author={Williams, D. A. and Hartquist, T. W. and Whittet, D. C. B.},
title={The ice threshold in molecular clouds: a diagnostic of the infrared radiation field},
journal={MNRAS},
fjournal={Monthly Notice of the Royal Astronomy Society},
volume=258,
pages={599-601},
year=1992,
doi={https://doi.org/10.1093/mnras/258.3.599}
}

@article{Williams2005,
author={Williams, D. A.},
title={Gas and dust in the interstellar medium},
journal={J. Phys.: Conf. Ser.},
fjournal={Journal of Physics: Conference Series},
volume=6,
pages={1-17},
year=2005,
doi={10.1088/1742-6596/6/1/001}
}


@article{Williams2011,
author={Williams, D. A. and Cieza, L. A.},
title={Protoplanetary Disks and Their Evolution},
journal={Annu. Rev. Astron. Astrophys.},
fjournal={Annual Review of Astronomy and Astrophysics },
volume=49,
pages={67-117},
year=2011,
doi={10.1146/annurev-astro-081710-102548}
}

@article{Wilburn1978,
author={Wilburn, D. R. and Bassett, W. A.},
title={Hydrostatic compression of iron and rlated compounds: an overview},
journal={Am. Min.},
fjournal={American Mineralogist},
volume=63,
pages={591-586},
year=1978,
doi={}
}


@article{Wing1977,
author={Wing, R. F. and Cohen, J. and Brault, J. W.},
title={Confirmation of the presence of iron hydride in sunspots and cool stars},
journal={ApJ.},
fjournal={Astrophysical Journal},
volume=216,
pages={659-664},
year=1977,
doi={https://ui.adsabs.harvard.edu/link_gateway/1977ApJ...216..659W/doi:10.1086/155507}
}



@article{Wright1987,
author={Wright, E. L.},
title={Long-Wavelength Absorption by Fractal Dust Grains},
journal={ApJ},
fjournal={The Astrophysical Journal},
volume=320,
pages={818-824},
year=1987,
doi={https://articles.adsabs.harvard.edu/pdf/1987ApJ...320..818W}
}

@article{Wurm2002,
author={Wurm, G. and Schnaiter, M.},
title={Coagulation as Unifiying Element for Interstellar Polarization},
journal={ApJ},
fjournal={The Astrophysical Journal},
volume=567,
pages={370-375},
year=2002,
doi={https://iopscience.iop.org/article/10.1086/338498}
}


@article{DeYoreo2015,
author={De Yoreo, J. J. and Gilbert, P. U. P. A. and Sommerdijik, N. A. J. M. and Penn, R. L. and Whitelam, S. and Joester, E. and Zhang, H. and Rimer, J. D. and Navtotsky, A. Banfield, J. F. and Wallace, A. F. and Michel, F. M. and Meldrum, F. C. and Colfen, H. and Dove, P. M.},
title={Crystallization by particle attachment in synthetic, biogeni, and geologic environment},
journal={Science},
fjournal={Science},
volume=349,
pages={6247},
year=2015,
doi={https://doi.org/10.1126/science.aaa6760}
}

@article{Yuan2021,
author={Yuan, L. and Steinle-Nuemann, G.},
title={The Helium Elemental and Isotopic Compositions of the Earth's Core Based on Ab Initio Simulations},
journal={JGR. Solid Earth},
fjournal={Journal of Geophysical Reserach: Solid Earth},
volume=126,
pages={e2021JB023106},
year=2021,
doi={https://doi.org/10.1029/2021JB023106}
}
